Learning to Attack Powergrids with DERs

In the past years, power grids have become a valuable target for cyber-attacks. Especially the attacks on the Ukrainian power grid has sparked numerous research into possible attack vectors, their extent, and possible mitigations. However, many fail to consider realistic scenarios in which time series are incorporated into simulations to reflect the transient behaviour of independent generators and consumers. Moreover, very few consider the limited sensory input of a potential attacker. In this paper, we describe a reactive power attack based on a well-understood scenario. We show that independent agents can learn to use the dynamics of the power grid against it and that the attack works even in the face of other generator and consumer nodes acting independently.

==> sections/env-task.tex <==
\section{Environment \& Task}
\label{sec:env-task}

% Env to train agents
In the following section, we describe the details of our voltage control environment that is used to train the \gls{DRL} agents.
% Two envs to test our hypotheses
To investigate our hypotheses, we consider two different variants of the environment that differ especially in their data distribution. 
% Env 1 short summary
\gls{ENV1} is the common denominator between the previously discussed publications. The goal is to perform actions so that existing voltage violations get cleared. The clearing of all violations also marks the end of the episode. 
% Env 2 short summary
\gls{ENV1} only considers clearing of existing violations. However, in the optimal case of voltage control, such violations get prevented from the start by using preventive action. Therefore, \gls{ENV2} considers a different data distribution where the agent not only sees voltage violations but also normal states of the power system. 

% Shared by both envs (before or after the two variants?)
Although differing in the details, both environments share most of their features, which we will describe in the following. 
% realistic Simbench time-series data sampled (+noise)
To sample from a realistic data distribution, we use the \simbench \cite{mei20} data set. \simbench consists of multiple network models, including a full year of time-series data for loads and generators in 15-minute-steps, resulting in about 35k samples. To prevent that these data points get sampled to often, we apply random noise of $\pm10\%$ to all setpoints during sampling. In our experiments, we use the \simbench model with code TODO, a TODO system with TODO buses, TODO generators, and TODO loads\todo{describe env}. After sampling, we use \pandapower \cite{thu18b} to run a powerflow calculation to determine the state of the power system.
% Constraints
The voltage band to satisfy is chosen as \(\pm \SI{5}{\%}\), as in related literature \citep{li2019coordination,Diao2019}. 
% Sensors
As observations we provide the learning agent with full information about the grid state, i.\,e., all bus voltages and all active/reactive power setpoints of loads and generators in the system. % ThW: zu viel? redundant? 
% Actuators
The actions of the agent are the reactive power setpoints of all generators in the system, which makes it a continuous actions space.
% Episode definition
The definition of an episode is one of the main differences between \gls{ENV1} and \gls{ENV2}.

% Env 1
% Based on literature (common denominator between publications; provide list of similar envs in literature!)
% Problem: Can the agents learn to maintain voltage constraints? 
In \gls{ENV1}, a single data point from the time-series data is sampled and used to set the grid state. Only samples with already existing voltage violations are used here. After sampling, the agent has multiple trials to clear the voltage violation. The episode ends in the case of success or after a maximum number of xy (TODO)\todo{trials?} trials. 

% Env 2
% Not only emergency but also preventing violations
% Episodes span multiple time steps
\gls{ENV2} aims to achieve more realistic training conditions for the agent. At the beginning of an episode, again, a random grid state is sampled from the time-series data, which is now allowed to contain non-violation states as well. After each step (observe, act, reward), the grid model is updated with the next data point in the time-series data to emulate a running power system. This way, the agent is not only trained to clear violations, but to completely prevent them in the optimal case. Since there is no clear success condition anymore, the episode ends after a fixed amount of xy\todo{n steps?} steps.

% Final words
% TODO: Both envs: Some data not sampled for testing to prevent memorizing -> better mention in experiments?
The reward function is exchangable to test different variants. All investigated reward functions are compatible with both environment variants and will be described in the following section.

% Weitere Ideen: (erstmal schauen wie viel Platz wir noch haben!)
% Bild oder Ablaufdiagramm der Env (was passiert wann in welcher Reihenfolge?)

% TODO:
% Wo details unterbringen? Anzahl steps, Netzmodell... Hier oder später in Experimentbeschreibung?
% Scaling erwähnen (eg to achieve more voltage violations, we use a scaling of xy in env 2)

